Parameter-Efficient Low-Resource Dialogue State Tracking by Prompt Tuning

Dialogue state tracking (DST) is an important step in dialogue management to keep track of users' beliefs. Existing works fine-tune all language model (LM) parameters to tackle the DST task, which requires significant data and computing resources for training and hosting. The cost grows exponentially in the real-world deployment where dozens of fine-tuned LM are used for different domains and tasks. To reduce parameter size and better utilize cross-task shared information, we propose to use soft prompt token embeddings to learn task properties. Without tuning LM parameters, our method drastically reduces the number of parameters needed to less than 0.5% of prior works while achieves better low-resource DST performance.

==> content/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}

Dialogue state tracking (DST) that extracts structured conversation progress in a list of slot-value pairs from unstructured dialogue utterances is an essential component of a dialogue system \cite{wang-lemon-2013-simple}. 
% For a dialogue system with a defined ontology, the DST component is expected to extract values for pre-defined slots \cite{chen2020schema,gao-etal-2020-machine}. 
% For example, we could extract the value of the slot ``price range'' as ``cheap'' from the conversation ``I want a cheap restaurant'', so that other downstream components like recommendation engine, information retrieval model could work with appropriate input to provide responses to the user. 
Recent works formulate DST as a conditional generation task \cite{gao-etal-2019-dialog,lin-etal-2020-mintl,peng-etal-2021-soloist}, where the dialogue history and a slot-specific question like ``what is the price range?'' are fed to models to generate slot values. This formulation enjoys the benefit of %flexibility and %ese attempts free some constrains of the DST task and the model 
generalizability to unseen domains and slot types beyond a defined dialogue ontology \cite{li-etal-2021-zero}. 

Despite its benefits, there are some non-trivial challenges when using a conditional generation model for DST. 
% Challenge 1: resources
Firstly, existing works fine-tune the entire LM for a new domain or task \cite{lin-etal-2021-zero,lee-etal-2021-dialogue}, requiring a significant amount of training time, system resources, and annotated data \cite{clarke-etal-2022-one,sauer-etal-2022-knowledge}. The resource-hungry issue is more severe in the real-world deployment where LMs tuned for different domains and tasks need to be trained and hosted, and a typical dialogue system has to serve dozens of such LMs \cite{maronikolakis-schutze-2021-multidomain,strubell-etal-2019-energy,lacoste2019quantifying}. This leads to a high cost of the development and service of dialogue systems and constrains offline deployment. In addition, limited data is available for a new domain or task. 
% Challenge 2: hard discrete questions
Secondly, the model is sensitive to the choice of manually created questions \cite{li-etal-2021-zero,gao-etal-2021-making}, and a single discrete question is far from a satisfying task representation. 
\looseness=-1
% Finally, there is no explicit signal for the generative model to learn task information and the model does not distinguish different segments of the input sequence to apply corresponding optimization.
% \di{This last sentence is a bit hard to understand.}

We propose a parameter-efficient DST model for low-resource settings as shown in \figref{fig:model}, which only needs to update 0.08\% of parameters compared with the previous best model, by keeping LM parameters frozen and introducing soft prompt tokens to represent task properties of different slots.
% first challenge
% While keeping parameters of the backbone LM frozen, we introduce soft prompt tokens to represent task properties of different slots with only 0.08\% of parameters updated compared with the previous best model. 
%Thus we can significantly reduce the resources needed for training and deployment.
\looseness=-1
%and initialize the soft prompt tokens with slot information like slot type, slot description and manually created slot questions. 

% second challenge
% \sarik{confused with this part do you mean using prompt in natural langugae format?}
More specifically, we introduce three techniques that are generalizable to other generative-based information extraction models. 
1) \textbf{Task-specific parameters}:
\textit{task prompt tokens} are introduced to specifically learn domain, slot and slot type information so that the model behaves according to the task; \textit{word-mapping prompt tokens} enable us to obtain task knowledge contained in natural language instruction and optimize human-created prompts with continuous embedding space. 
% third challenge
2) \textbf{Task metadata in objective}:
we introduce the reiteration technique in the target sequence in order to include explicit task signals in the text generation objective. 
3) \textbf{Distinguishing segments}:
segment embeddings help the model identify the prompt segment, dialogue speakers, and question partition.
\looseness=-1
% broader impact
% All the newly introduced techniques can be generalized to other information extraction tasks that use generative models for better performance.
% \sarik{maybe change this paragraph in such a way that exactly shows in which parts are your contributions? (like abstract keyword and then explain it. (long paragraph) seems like you wanted to explain whole your paper here :) maybe mention those parts in Figure 1 )}

\begin{figure*}[thp]
    \centering
    \includegraphics[width=0.94\textwidth]{figs/model.pdf}
    \vspace{-2mm}
    \caption{Model design. Snow icon indicates non-trainable parameters. Absolute positional embeddings are added together with segment embeddings and sequence embeddings, we omit it for simplicity in the illustration.}
    \label{fig:model}
    \vspace{-6mm}
\end{figure*}

Experiments on MultiWOZ 2.0 show that our method achieves better performance on low-resource DST with orders of magnitude fewer parameters. We further conduct ablation studies, error analysis, and examine the semantic information shown in the prompt tokens. We observe that our model is more specialized in predicting categorical slot values, is more conservative for slots with free output space and introduces more hallucination errors for categorical slots.
\looseness=-1
% \sviolet{would be nice to have a list of contribution. Can be brief.}

==> tables/domain_adaptation.tex <==
\begin{table*}[ht]
\begin{center}
%\resizebox{\linewidth}{!}{
{
\small
\setlength\tabcolsep{2pt}
\begin{tabular}{lr
rrr
rrr
rrr
rrr
rrr}
\toprule
\multirow{2}{*}{Model} 
& \multirow{2}{*}{\# Params}
& \multicolumn{3}{c}{Attraction} 
& \multicolumn{3}{c}{Hotel}
& \multicolumn{3}{c}{Restaurant}
& \multicolumn{3}{c}{Taxi}
& \multicolumn{3}{c}{Train}
\\
& & 1\% & 5\% & 10\% & 1\% & 5\% & 10\% & 1\% & 5\% & 10\% & 1\% & 5\% & 10\% & 1\% & 5\% & 10\% \\ 
% \cmidrule{2-17}
TRADE &
&35.88&57.55&63.12
&19.73&37.45&41.42
&42.42&55.7&60.94
&63.81&66.58&70.19
&59.83&69.27&71.11
\\
DSTQA &
&---&\textbf{70.47}&\textbf{71.60}
&---&50.18&53.68
&---&58.95&\textbf{64.51}
&---&70.90&74.19
&---&70.35&74.50
\\
Li et al. & 355M 
& 53.04 & 59.47 & 65.04 
& 33.88 & 48.56 & 51.25
& 42.2 & 53.67 & 55.00
& 62.05 & 69.29 & 70.57
& 68.14 & 74.16 & 76.42 
\\
T5DST & 60M 
& \textbf{58.77} & 65.72 & 69.54 
& \textbf{43.07} & \textbf{50.71} & \textbf{54.86}
& \textbf{57.63} & \textbf{61.86} &63.47 
&\textbf{70.12} & \textbf{73.67} & \textbf{74.70}
&\textbf{70.82} & \textbf{74.18} & \textbf{77.57}
\\
\midrule
Old & 390K 
&&&
& 29.61 &  &
& 31.08 &  &
& 59.82 &  &
&  &  &
\\
Ours & 390K 
&&&
&  &  &
& 43.25 & 53.98 &
&  &  &
&  &  &
\\
\bottomrule
\end{tabular}
%}
}

\caption{
Domain adaptation, JGA. All metrics are higher the better.
}
\label{table:overall}
\end{center}
%\vspace{-5mm}
\end{table*}

==> tables/fewshot_hotel.tex <==
\begin{table*}[ht]
\begin{center}
%\resizebox{\linewidth}{!}{
{
% \small
\setlength\tabcolsep{2pt}
\begin{tabular}{l
rrrr
|rrrr}
\toprule
\multirow{2}{*}{Model} 
& \multicolumn{4}{c|}{1\%}
& \multicolumn{4}{c}{5\%}
\\
& JGA & SA & E-JGA & E-SA & JGA & SA & E-JGA & E-SA \\ \hline
% \cmidrule{2-17}

\citet{li2021zero} 
& 19.60 & 64.61 & - & -
& 30.71 & 82.25 & - & - \\
\citet{lin2021leveraging} 
& 18.63 & - & - & -
& 38.76 & - & - & - \\
\midrule
Ours 
& 18.65 & 76.12 & 13.41 & 61.39
& 31.47 & 87.52 & 36.29 & 77.71
\\ \hline
- Prefix prompts 
& 12.93 & 74.61 & 8.76 & 52.53 & - & - & - & - \\
- Question prompts
& 16.61 & 73.95 & 4.68 & 48.98 & - & - & - & - \\
\bottomrule
\end{tabular}
%}
}

\caption{
Few-shot learning result on target domain hotel. 
JGA/SA representing Joint Goal Accuracy/Slot Accuracy for all slots. E-JGA/E-SA means the JGA/SA metrics for the slots with values, if the ground-truth of a slot is empty, the prediction result of such a slot is not included.
All metrics are higher the better. We reproduce the result of the two baselines by rerunning their codebases on MultiWOZ 2.1 and our few-shot experimental setting. 
}
\label{table:overall}
\end{center}
%\vspace{-5mm}
\end{table*}

==> tables/fewshot_v1.tex <==
\begin{table*}[th]
\begin{center}
\resizebox{\linewidth}{!}{
{
% \small
\setlength\tabcolsep{2pt}
\begin{tabular}{lr
HHccc
HHccc
HHccc
HHccc
HHccc}
\toprule
\multirow{2}{*}{Model} 
& \multirow{2}{*}{\# Params}
& \multicolumn{5}{c}{Attraction} 
& \multicolumn{5}{c}{Hotel}
& \multicolumn{5}{c}{Restaurant}
& \multicolumn{5}{c}{Taxi}
& \multicolumn{5}{c}{Train}
\\
& & 10 & 20 & 1\% & 5\% & 10\% & 10 & 20 & 1\% & 5\% & 10\% & 10 & 20 & 1\% & 5\% & 10\% & 10 & 20 & 1\% & 5\% & 10\% & 10 & 20 & 1\% & 5\% & 10\% \\ 
% \cmidrule{2-17}
\midrule
TRADE &
&---&---&---&52.19&58.46
&---&---&---&31.93&41.29
&---&---&---&47.31&53.65
&---&---&---&59.03&60.51
&---&---&---&48.82&59.65
\\
DSTQA &
&---&---&---&51.58&61.77
&---&---&---&33.08&\textbf{49.69}
&---&---&---&35.33&54.27
&---&---&---&58.25&59.35
&---&---&---&50.36&61.28
\\
Li et al. & 335M
&27.09&35.63&42.18&49.13&60.85 
&15.15&19.44&24.04&37.88&46.47
&22.82&25.68&30.70&49.75&\textbf{58.50}
&50.99&57.47&58.26&\textbf{61.68}&\textbf{69.23}
&27.42&39.27&45.32&\textbf{71.69}&73.45
\\
T5DST & 60M
&&&40.68&52.12&60.13
&&&18.63&\textbf{38.76}&46.13
&&&29.47&\textbf{53.32}&58.44
&&&58.19&59.23&69.03
&&&43.93&69.27&69.48
\\
\midrule
% Old & 110K %370K
% & 44.22 & 55.17 & 63.61
% & 26.49 & 38.24 & 45.60
% & 31.77 & 50.81 & 55.79
% & 60.33 & 57.47 & 63.00
% & 51.08 & 67.25 & 75.00
% \\
Ours & 271K
&&& \textbf{47.28} & \textbf{56.99} & \textbf{63.61}
&&& \textbf{33.01} & 38.24 & 45.60
&&& \textbf{34.40} & 50.81 & 55.79
&&& \textbf{60.33} & 61.63 & 63.00
&&& \textbf{52.05} & 69.51 & \textbf{75.00}
\\
% Ours (4 prefix) & 627K
% & 37.47 & 54.7 &
% & 25.33 & & % check
% & 25.93 & & % check
% & 61.00 & &
% & 22.61 & & % check
% \\
% Ours (1 prefix) & 73K
% & 36.55 &&
% \\ 
% Ours (0 prefix) & 20K 
% & 24.04 &&
% \\
% Old (4 prefix)  & 627K 
% & 22.86 & 46.65 & 
% & 25.30 &  & 
% % & 25.3 & 21.77 & 
% & 20.53 & 27.43 &
% & 61.73 & 61.99 &
% & 16.35 & 20.88 &
% \\
% Old (1 prefix) & 73K 
% & 19.20 & 31.63 &
% & 18.65 & 31.47 &
% & & &
% & 16.62 & 37.40 &
% & 16.62 & &
% \\
% Old (0 prefix) & 20K 
% &&&
% & 6.79 & 16.86 &
% &&&
% &&&
% &&&
% \\
\bottomrule
\end{tabular}
}
}

\caption{
Few shot generalization performance on five target domains. We report Joint Goal Accuracy (JGA), which is higher the better. 271K is the average parameter count across domains, detailed information is provided in \secref{app:detailed_parameter_count}.
% E-JGA/E-SA means the JGA/SA metrics for the slots with values, if the ground-truth of a slot is empty, the prediction result of such a slot is not included.
\derek{I'm running experiments with fewer shot: 1, 5, and 10 conversations}
}
\label{table:overall}
\end{center}
%\vspace{-5mm}
\end{table*}

==> tables/zeroshot.tex <==
\begin{table}[ht]
\begin{center}
%\resizebox{\linewidth}{!}{
{
\small
\setlength\tabcolsep{2pt}
\begin{tabular}{lr
r
r
r
r
r}
\toprule
\multirow{1}{*}{Model} 
& \multirow{1}{*}{\# Params}
& \multicolumn{1}{c}{Attr.} 
& \multicolumn{1}{c}{Hotel}
& \multicolumn{1}{c}{Rest.}
& \multicolumn{1}{c}{Taxi}
& \multicolumn{1}{c}{Train}
\\
% & & 1\% & 5\% & 10\% & 1\% & 5\% & 10\% & 1\% & 5\% & 10\% & 1\% & 5\% & 10\% & 1\% & 5\% & 10\% \\ 
% \cmidrule{2-17}
\midrule 
TRADE &
& 20.06 & 14.20 & 12.59 & 59.21 & 22.39
\\
MA-DST &
& 22.46 & 16.28 & 13.56 & 59.27 & 22.76
\\
SUMBT &
& 22.60 & 19.80 & 16.50 & 59.50 & 22.50
\\
Li et al. & 355M
& 31.31 & 24.41 & 26.17 & 59.61 & 29.07
\\
\midrule
Li et al Our Run & 355M
& 23.18 & 14.81 & 19.70 & 50.54 & 23.00
\\
Prompt & 370K
& 21.33 & 0.34 & 14.70 & 58.36 & 18.69
\\
LM + Prompt, Old & 355M
& & 16.45 & 17.27 & 57.02 &
\\
LM + Prompt & 355M
& & 18.95 & 18.69 & &
\\
\bottomrule
\end{tabular}
%}
}

\caption{
Zero-shot. MultiWoz 2.1
}
\label{table:zeroshot}
\end{center}
%\vspace{-5mm}
\end{table}
